AdaSAM: Boosting Sharpness-Aware Minimization with Adaptive Learning Rate and Momentum for Training Deep Neural Networks

Sharpness aware minimization (SAM) optimizer has been extensively explored as it can generalize better for training deep neural networks via introducing extra perturbation steps to flatten the landscape of deep learning models. Integrating SAM with adaptive learning rate and momentum acceleration, dubbed AdaSAM, has already been explored empirically to train large-scale deep neural networks without theoretical guarantee due to the triple difficulties in analyzing the coupled perturbation step, adaptive learning rate and momentum step. In this paper, we try to analyze the convergence rate of AdaSAM in the stochastic non-convex setting. We theoretically show that AdaSAM admits a $\mathcal{O}(1/\sqrt{bT})$ convergence rate, which achieves linear speedup property with respect to mini-batch size $b$. Specifically, to decouple the stochastic gradient steps with the adaptive learning rate and perturbed gradient, we introduce the delayed second-order momentum term to decompose them to make them independent while taking an expectation during the analysis. Then we bound them by showing the adaptive learning rate has a limited range, which makes our analysis feasible. To the best of our knowledge, we are the first to provide the non-trivial convergence rate of SAM with an adaptive learning rate and momentum acceleration. At last, we conduct several experiments on several NLP tasks, which show that AdaSAM could achieve superior performance compared with SGD, AMSGrad, and SAM optimizers.

==> 7-bio.tex <==
\begin{IEEEbiography}
[{\includegraphics[height=1.16in,clip,keepaspectratio]{pho/haosun.jpg}}]
{Hao Sun} is working toward the doctoral degree at the University of Science and Technology of China, Hefei, China. His research interests include distributed machine learning and optimization.
\end{IEEEbiography}




\begin{IEEEbiography}
[{\includegraphics[height=1.16in,clip,keepaspectratio]{pho/shenli.jpg}}]
{Li Shen} received his Ph.D. in school of mathematics, South China University of Technology in 2017. He is currently a research scientist at JD Explore Academy, China. Previously, he was a research scientist at Tencent AI Lab, China. His research interests include theory and algorithms for large scale convex/nonconvex/minimax optimization problems, and their applications in statistical machine learning, deep learning, reinforcement learning, and game theory.
\end{IEEEbiography}


\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pho/zhongqihuang.jpg}}]
{Qihuang Zhong} is currently pursuing a Ph.D. degree in Artificial Intelligence from the School of Computer Science, Wuhan University. His research interests mainly include natural language processing, image processing and machine learning. He has authored or co-authored several papers at top conferences and international journals.
\end{IEEEbiography}



\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pho/dingliang.jpg}}]
{Liang Ding} received Ph.D. from the University of Sydney. He is currently an algorithm scientist with JD.com and leading the NLP research group at JD Explore Academy. He works on deep learning for NLP, including language model pretraining, language understanding, generation, and translation. He published over 30 research papers in NLP/AI, including ACL, EMNLP, NAACL, COLING, ICLR, AAAI, SIGIR, and CVPR, and importantly, some of his works were successfully applied to the industry. He served as Area Chair for ACL 2022 and Session Chair for SDM 2021 and AAAI 2023. He won many AI challenges, including SuperGLUE/ GLUE, WMT2022, IWSLT 2021, WMT 2020, and WMT 2019.
\end{IEEEbiography}



\begin{IEEEbiography}
[{\includegraphics[height=1.16in,clip,keepaspectratio]{pho/chenshixiang.jpeg}}]
{Shixiang Chen}  is currently an Algorithm Scientist at JD Explore Academy. He was a postdoctoral associate in the Department of Industrial  \& Systems Engineering at Texas A\&M University (TAMU), with Prof. Alfredo Garcia and Prof. Shahin Shahrampour. He received Ph.D. degree in Systems Engineering and Engineering Management from The Chinese University of Hong Kong in July, 2019 and B.S. degree in Mathematics from Nanjing University in 2015. His current research interests include design and analysis of optimization algorithms, and their applications in machine learning and signal processing; non-convex optimization; the theory and methods for distributed networking.
\end{IEEEbiography}


\begin{IEEEbiography}
[{\includegraphics[height=1.16in,clip,keepaspectratio]{pho/JingweiSun.jpg}}]
{Jingwei Sun} is currently an associate researcher in school of computer science and technology, University of Science and Technology of China. His research interests include high performance computing, parallel algorithms, performance profiling and modeling.
\end{IEEEbiography}



\begin{IEEEbiography}
[{\includegraphics[height=1.16in,clip,keepaspectratio]{pho/lijing.jpg}}]
{Jing Li} received the bachelor’s, master’s, and Ph.D. degrees in computer science from the University of Science and Technology of China (USTC), in 1987, 1990, and 1993, respectively. He is currently a Professor with the School of Computer Science and Technology, USTC. He published more than 80 articles in high-profile domestic and international academic journals. His recent research interests include distributed systems, cloud computing, and mobile computing. In the last few years, he was mainly engaged in the promotion and application of software technology, large-scale network systems, and the research and development of distributed algorithms. He is a Senior Member of the CCF.
\end{IEEEbiography}



\begin{IEEEbiography}
[{\includegraphics[height=1.16in,clip,keepaspectratio]{pho/guangzhongsun.jpg}}]
{Guangzhong Sun} is a professor with the School of Computer Science and Technology, University of Science and Technology of China, Hefei, China. He is also a member of National High Performance Computing Center (Hefei) and the principal investigator of Algorithm and Data Application (Ada) Research Group. His research interests include high performance computing, algorithm optimizations, and data processing.
\end{IEEEbiography}


\begin{IEEEbiography}
[{\includegraphics[height=1.16in,clip,keepaspectratio]{pho/DachengTao.png}}]
{Dacheng Tao} (Fellow, IEEE) is currently the president of JD Explore Academy and a Senior Vice President of JD.com. He is also an advisor and chief scientist of the digital science institute at the University of Sydney. He mainly applies statistics and mathematics to artificial intelligence and data science. His research interests range across computer vision, data science, image processing, machine learning, and video surveillance. His research results have been presented in one monograph and 500+ publications in prestigious journals and at prominent conferences, such as IEEE T-PAMI, T-NNLS, T-IP, JMLR, IJCV, NIPS, ICML, CVPR, ICCV, ECCV, ICDM, and ACM SIGKDD, with several Best Paper awards, such as the Best Theory/Algorithm Paper Runner Up Award at IEEE ICDM07, the Best Student Paper Award at IEEE ICDM13, the Distinguished Student Paper Award at the 2017 IJCAI, the 2014 ICDM 10-Year Highest-Impact Paper Award, and the 2017 IEEE Signal Processing Society Best Paper Award. He was a recipient of the 2015 Australian Scopus-Eureka Prize, the 2015 ACS Gold Disruptor Award, and the 2015 UTS Vice-Chancellor’s Medal for Exceptional Research. He is a Fellow of AAAS, OSA, IAPR, and SPIE. 
\end{IEEEbiography}
